Tromino: Demand and DRF Aware Multi-Tenant Queue Manager for Apache Mesos Cluster

Apache Mesos, a two-level resource scheduler, provides resource sharing across multiple users in a multi-tenant cluster environment. Computational resources (i.e., CPU, memory, disk, etc. ) are distributed according to the Dominant Resource Fairness (DRF) policy. Mesos frameworks (users) receive resources based on their current usage and are responsible for scheduling their tasks within the allocation. We have observed that multiple frameworks can cause fairness imbalance in a multiuser environment. For example, a greedy framework consuming more than its fair share of resources can deny resource fairness to others. The user with the least Dominant Share is considered first by the DRF module to get its resource allocation. However, the default DRF implementation, in Apache Mesos' Master allocation module, does not consider the overall resource demands of the tasks in the queue for each user/framework. This lack of awareness can result in users without any pending task receiving more resource offers while users with a queue of pending tasks starve due to their high dominant shares. We have developed a policy-driven queue manager, Tromino, for an Apache Mesos cluster where tasks for individual frameworks can be scheduled based on each framework's overall resource demands and current resource consumption. Dominant Share and demand awareness of Tromino and scheduling based on these attributes can reduce (1) the impact of unfairness due to a framework specific configuration, and (2) unfair waiting time due to higher resource demand in a pending task queue. In the best case, Tromino can significantly reduce the average waiting time of a framework by using the proposed Demand-DRF aware policy.

==> 1a_motivation.tex <==
\section{motivation}
Even though Apache Mesos and its DRF based allocation module is well intentioned but in our \fixme{previous work}\cite{} we have identified how resource allocation and fairness can be hindered due to different properties of frameworks like offer refusal period, resource holding period, task arrival rate, second level scheduling policy etc. Figure \ref{fig_moti_scylla_aurora} and \ref{fig_moti_scylla_marathon} shows how resource distribution and fairness went imbalanced in a Mesos cluster. Aurora in Figure \ref{fig_moti_scylla_aurora} and Scylla in Figure \ref{fig_moti_scylla_marathon} is suffering from unfair resource distribution. 

We have developed one queue manager, \textit{Tromino}, which is aware of DRF and dominant share of each framework in the cluster. Tromino controls the awaiting task queue of each framework and releases tasks based on the dominant share for better fairness utilization. We have also considered situation where few framework in a cluster have higher demands compared to others and releasing tasks only based on Dominant Share may bring better fairness but increases the waiting time of tasks. We have implemented scheduling policies based on Dominant Share or and Demands. 


Key contributions of our work is as following:
\begin{itemize}
\item We have designed and developed a queue manager , Tromino, on top of Apache Mesos scheduler which keeps track of incoming tasks of all connected frameworks and current resource consumption of them. 
\item “Tromino” can gather resource demand and consumption information from awaiting queue and Mesos Master respectively to control the task dispatching, based on the current demand.
\item We have shown how our demand aware scheduling on top of Mesos’s default DRF aware, can bring better throughput and fair waiting time.
\item We have also proposed and show how different policies of task disbursements based on the demand, dominant share and both produces fairness results for different case scenarios. 
\end{itemize}


\begin{figure*}%
	\captionsetup[subfigure]{justification=centering}
	\centering
    \subfloat[{\it Scylla and Aurora are competing for resources in a Mesos cluster. %Scylla gets significantly more resources in the beginning. Aurora is able to launch its tasks only after Scylla is done launching all its tasks. Aurora's tasks are starving for resources when launched along with Scylla.
    } 
    ]{{\includegraphics[width=0.30\linewidth]
    {images/moti_scylla_aurora.pdf}  
    \label{fig_moti_scylla_aurora}
    }}
%
%
    \subfloat[{\it  Scylla and Marathon are competing for resources in a Mesos cluster.
    %Marathon gets significantly more resources and is thus able to launch several more tasks than Scylla. Scylla's tasks face long wait times due to unfair distribution
    }]
{{\includegraphics[width=0.30\linewidth]
    {images/moti_scylla_marathon.pdf}
    \label{fig_moti_scylla_marathon}
    }}
%  
%
    \subfloat[{\it  Scylla, Marathon and Aurora are competing for resources in a Mesos cluster.}]
{{\includegraphics[width=0.30\linewidth]
    {images/moti_scylla_marathon_aurora.pdf}
    \label{moti_scylla_marathon_aurora}
    }}
%
%
\caption{Resource Fairness : }
\end{figure*}

==> 4_experimentalSetup.tex <==
\section {experimental setup}

